Programmatic Imitation Learning from Unlabeled and Noisy Demonstrations

Imitation Learning (IL) is a promising paradigm for teaching robots to perform novel tasks using demonstrations. Most existing approaches for IL utilize neural networks (NN), however, these methods suffer from several well-known limitations: they 1) require large amounts of training data, 2) are hard to interpret, and 3) are hard to repair and adapt. There is an emerging interest in programmatic imitation learning (PIL), which offers significant promise in addressing the above limitations. In PIL, the learned policy is represented in a programming language, making it amenable to interpretation and repair. However, state-of-the-art PIL algorithms assume access to action labels and struggle to learn from noisy real-world demonstrations. In this paper, we propose PLUNDER, a novel PIL algorithm that integrates a probabilistic program synthesizer in an iterative Expectation-Maximization (EM) framework to address these shortcomings. Unlike existing PIL approaches, PLUNDER synthesizes probabilistic programmatic policies that are particularly well-suited for modeling the uncertainties inherent in real-world demonstrations. Our approach leverages an EM loop to simultaneously infer the missing action labels and the most likely probabilistic policy. We benchmark PLUNDER against several established IL techniques, and demonstrate its superiority across five challenging imitation learning tasks under noise. PLUNDER policies achieve 95% accuracy in matching the given demonstrations, outperforming the next best baseline by 19%. Additionally, policies generated by PLUNDER successfully complete the tasks 17% more frequently than the nearest baseline.

==> em_fig.tex <==
    % figure showing the progress of EM loop and how the quality of the programs improve
    \def\leftscalefactor{0.22}
    \def\rightscalefactor{0.2}
    \begin{figure}[h]
        \centering
        \begin{minipage}[c]{\leftscalefactor\textwidth}
            \centering
                \includegraphics[width=1.25\textwidth]{figs/0-8-graph copy.png}
        \end{minipage}
                \hfill
        \begin{minipage}[c]{\rightscalefactor\textwidth}
        \footnotesize
          $\guard_{\ha{ACC},\ha{CON}}\!:=\!
     \stx{stochastic}(90)   \\
    \guard_{\ha{CON},\ha{DEC}}\!:=\!
    \stx{stochastic}(90) $
        \end{minipage}
                \\[1mm]
        \begin{minipage}[c]{\leftscalefactor\textwidth}
            \centering
                \includegraphics[width=1.25\textwidth]{figs/1-8-graph copy.png}
        \end{minipage}
                \hfill
        \begin{minipage}[c]{\rightscalefactor\textwidth}
        \footnotesize
$\guard_{\ha{ACC},\ha{CON}}:= \\[-0.2mm]
     {\stx{flp}(\stx{lgs}(v\!-\!v_{\max},5.1, 0.3))}   \\
    \guard_{\ha{CON},\ha{DEC}}:=\\[-0.2mm]
   {\stx{flp}(\stx{lgs}(p, 107.0, 0.08)) }$
        \end{minipage}
                \\[1mm]
        \begin{minipage}[c]{\leftscalefactor\textwidth}
            \centering 
                \includegraphics[width=1.25\textwidth]{figs/3-8-graph copy.png}
        \end{minipage}
                \hfill
        \begin{minipage}[c]{\rightscalefactor\textwidth}
        \footnotesize
            $\guard_{\ha{ACC},\ha{CON}}:= \\[-0.2mm]
     {\stx{flp}(\stx{lgs}(v\!-\!v_{\max},0.9, 0.8))}   \\
    \guard_{\ha{CON},\ha{DEC}}:=\\[-0.2mm]
   {\stx{flp}(\stx{lgs}(p, 101.5, 0.09)) }$
        \end{minipage}
                \\[1mm]
        \begin{minipage}[c]{\leftscalefactor\textwidth}
            \centering
                \includegraphics[width=1.25\textwidth]{figs/4-8-graph copy.png}
        \end{minipage}
                \hfill
        \begin{minipage}[c]{\rightscalefactor\textwidth}
        \footnotesize
            $\guard_{\ha{ACC},\ha{CON}}:= \\[-0.2mm]
     {\stx{flp}(\stx{lgs}(v\!-\!v_{\max},0.1, 1.1))}   \\
    \guard_{\ha{CON},\ha{DEC}}:=\\[-0.2mm]
   {\stx{flp}(\stx{lgs}(}\\[-0.2mm] 
  {\stx{distStp}(p)-\stx{distTrv}(v,a_{\min}), 3.2, 0.1)) }$
        \end{minipage}
                \\[1mm]
        \begin{minipage}[c]{\leftscalefactor\textwidth}
            \centering
                \includegraphics[width=1.25\textwidth]{figs/5-8-graph copy.png}
        \end{minipage}
                \hfill
        \begin{minipage}[c]{\rightscalefactor\textwidth}
        \footnotesize
            $\guard_{\ha{ACC},\ha{CON}}:= \\[-0.2mm]
     {\stx{flp}(\stx{lgs}(v\!-\!v_{\max},0.1, 0.9))}   \\
    \guard_{\ha{CON},\ha{DEC}}:=\\[-0.2mm]
   {\stx{flp}(\stx{lgs}(p+\stx{distTrv}(v,a_{\min}),}\\[-0.2mm] \hspace{3mm} {\;\;\;\;\;\;\;\;\;\;\;\;\;\; 99.4, 0.4)) }$
        \end{minipage}
                

        \caption{
        EM Loop Progression: candidate programs at each iteration (right) and corresponding distribution of high-level actions (left). 
        %\kia{can we get rid of the negative values without effecting the story?} 
        %\jiayi{We can also show programs and trajectories separately instead of side-by-side.}
        } 
        \label{fig:em}
    \end{figure}


==> history.tex <==
CONTENTS OF THIS FILE ARE NOT USED IN THE PDF


%Consider a hypothetical robotic tournament, wherein robots partake in a competition on a linear 100-meter track. The objective of each robot is to cross the finish line expeditiously and come to a halt in the closest possible proximity to the line.

%Autonomous robots, on the other hand, are controlled by programmatic action selection policies (ASP) that model their behaviors as high-level state transition systems, which specify the conditions for state transitions. 
%These conditions, referred to as \textit{guarding conditions} or \textit{transition guards}, determining the transition from state $x\in H$  to state $y\in H$, and are denoted by $\guard_{x,y}$. The guarding conditions are defined based on the \textit{low-level state} of the robot as observed by the robot itself.
%
%In this example, the low-level state of each robot is represented by a tuple $L:=(p,v,a)$, which captures its current position on the line, velocity, and acceleration. At each time-step, the robot's acceleration is added to its current velocity, i.e., $v_{t+1} = v_t + a$. Consequently, a positive acceleration value results in an increase in velocity, while a negative acceleration value leads to a decrease in velocity.

%

% Similarly, the robot's velocity is constrained by a known constant $v_{\max}>0$, i.e., $0\leq v\leq v_{\max}$ at all times.

%
%Each attempt involved initiating the robot at rest and subsequently accelerating it by manipulating the joy-stick until the velocity approached $v_{\max}$ ($t\approx 50s$). The joy-stick was then released to maintain a constant velocity for a brief duration, after which the robot was decelerated by pulling the joy-stick until it came to a stop ($t\approx75s$).
% %

%
%The presented trajectories are color-coded according to the user's action, where red indicates acceleration (\textcolor{my_red}{$\ha{ACC}$}), cyan indicates maintaining a constant velocity (\textcolor{my_cyan}{$\ha{CON}$}), and blue indicates deceleration (\textcolor{my_blue}{$\ha{DEC}$}). However, such high-level labels are not typically available and are difficult to obtain, and are only shown in this context for the purpose of presentation.

%The presented trajectories demonstrate significant variation in the user's decision-making regarding state transitions. For instance, one trajectory indicates a conservative behavior with an earlier switch from acceleration to constant velocity, resulting in significantly lower maximum velocity reached compared to other trajectories.
%Additionally, in \autoref{subfig:demo_acc}, the acceleration trajectories exhibit small but continuous variations, attributed to the inherent noise in the robot's actuation module. Such variations and noises in low-level human-provided demonstrations are widespread and require substantial manual intervention to eliminate. 


%Existing Learning from Demonstration (LfD) approaches are ineffective in handling such noisy demonstrations \kia{more elaboration?}. To address this challenge, we propose \algname{}, a novel approach for learning programmatic robot policies from such noisy and unlabeled demonstration trajectories.


%Our objective is to generate a concise probabilistic program that captures the underlying intention of the provided trajectories. Probabilistic programs are a suitable choice for such policies because \kia{???}.
%
Specifically, our focus is on probabilistic programs that incorporate probabilistic coin-flips instead of Boolean predicates and a logistic S-shaped curve instead of exact numerical inequalities.
%
As a result, the language we use to derive programs includes two operators, namely $\stx{flp}$ and $\stx{lgs}$. The $\stx{flp}(p)$  generates a Boolean value, which is true with probability $p$ and false with probability $1-p$. 
Using the $\stx{flp}$ function, exact inequalities in the programs, 
such as $e>x_0$, are replaced with approximate versions, such as 
$\stx{flp}(\stx{lgs}(e,x_0,k))$, where $\stx{lgs}(e,x_0,k)$ maps the difference between the values of $e$ and $x0$ to a value in the range $[0,1]$ in a smooth and continuous manner. The parameter $k$ determines the sharpness of the resulting sigmoid curve; the larger $k$ represents a more rapid increase of the output value as the value of expression $e$ is approaching $x_0$.




For example, the expression $\stx{flp(lgs(v_{\max} - v, 0 , 10))}$ is evaluated to true with a certain probability that rapidly grows when $\stx{v_{\max}-v}$ gets closer to $0$. Such logistic functions are commonly used in statistics and machine learning for binary classification problems, and here too, we use them to capture the natural uncertainties that \kia{????}.



\begin{comment}
\begin{tabular}{l|lll}
    \toprule
    & \multicolumn{3}{c}{\textbf{Log Observation Likelihood}}\\
    & \tabheader{c}{Target} & \tabheader{c}{Highway} & \tabheader{c}{Merge}\\
    \midrule
    M-SYNTH & -2.192 & -1.479 & -0.743\\
    M-SYNTH+ & -1.123 & -1.782 & -0.653\\
    BC & -4.930 & -1.788 & -0.116\\
    BC+ & -1.208 & -1.101 & -1.296\\
    \fixme{GAIL?} & - & - & -\\
    \algname{} & \textbf{-0.779} & \textbf{-0.536} & \textbf{0.257}\\
    \midrule
    \emph{EM-Truth} & \emph{-0.783} & \emph{-0.621} & \emph{0.272}\\
    \emph{Ground Truth} & \emph{-0.796} & \emph{0.599} & \emph{0.896}\\
    \bottomrule
\end{tabular}
\end{comment}

==> related.tex <==



\section{Related Work} 
\label{sec:related}
This paper is related to an extensive body of research on learning frameworks for sequential decision-making. In this section, we briefly summarize existing methodologies and compare our approach against them.
%
\paragraph*{Imitation Learning}
Imitation Learning (IL) is a framework for learning the agent's desired behaviors from human demonstrations~\cite{9927439}. 
%
Unlike Reinforcement Learning (RL) techniques, IL does not require access to any explicit reward signals. 
%
 While RL has been successful in solving many complex tasks~\cite{silver2017mastering,vinyals2019grandmaster,akkaya2019solving,sutton2018reinforcement}, it can be challening, even for experts, to devise reward objectives that lead to desired agent behaviors~\cite{boularias2011relative}. 
%in alternative approaches, namely the reinforcement learning (RL) framework, which require explicit reward signals. While RL has been highly successful in solving numerous complex tasks~\cite{silver2017mastering,vinyals2019grandmaster,akkaya2019solving,sutton2018reinforcement}, it can be challenging, even for experts, 
%
Popular IL solutions include Behavior Cloning (BC)~\cite{ross2011reduction, daftry2017learning, bojarski2016end, giusti2015machine, pomerleau1991efficient}, which aims to learn a function that directly maps observations to actions, and Inverse Reinforcement Learning (IRL)~\cite{ng2000algorithms,ziebart2008maximum,abbeel2004apprenticeship}, which seeks to infer the intrinsic reward structure underlying the provided trajectories, then uses RL for policy inference. 
%
IRL often requires more sophisticated algorithms and significantly more data than BC. 
%
Our approach in \algname{} is more aligned with the BC setup where a quick and relatively accurate mimicry of expert behavior is needed without diving deep into the underlying motivations aiming at either enhancing the expert performance or transferring the learned knowledge to related tasks~\cite{brown2019extrapolating}. 
%
There also works that draw insight from both BC and IRL, for instance, Generative Adversarial Imitation Learning (GAIL)~\cite{gail} is an imitation learning method in which a policy network and a discriminator network are jointly trained through an adversarial process~\cite{goodfellow2014generative}. 



%modeling the demonstrator's intentions and allowing generalization to states not visited during the demonstration~\cite{brown2019extrapolating}.
%
%However, IRL often requires more sophisticated algorithms and significantly more data than BC to reliably infer the underlying reward structures. 
%
%Our approach in \algname{} is more aligned with the BC setup where a quick and relatively accurate mimicry of expert behavior is needed without diving deep into the underlying motivations aiming at enhancing the expert performance or transferring the learned knowledge to related tasks. 
%
%BC has proven effective in facilitating end-to-end supervised learning for autonomous robots operating in cluttered and complex environments, such as forest trails~\cite{giusti2015machine} or parking lots and unpaved roads~\cite{bojarski2016end}. 





\newpage

%Many learning frameworks use an explicit reward structure to analyze the agent's self-supervised explorations and devise an optimal policy. Such reinforcement learning (RL) techniques have been highly successful in solving numerous complex tasks~\cite{silver2017mastering,vinyals2019grandmaster,akkaya2019solving,sutton2018reinforcement},  however, even for experts, it can be challenging to devise reward objectives that lead to desired agent behaviors in complex domains~\cite{boularias2011relative}.
%
%Imitation Learning (IL)~\cite{9927439} approaches address this challenge by attempting to learn the desired policy without requiring access to a reward structure.
%
%Popular IL methods include Behavioral Cloning (BC)~\cite{ross2011reduction, daftry2017learning, bojarski2016end, giusti2015machine, pomerleau1991efficient}, which aims to learn a function that directly maps observations to actions, and Inverse Reinforcement Learning (IRL)~\cite{ng2000algorithms,ziebart2008maximum,abbeel2004apprenticeship}. IRL seeks to infer the intrinsic reward structure underlying the provided trajectories, modeling the demonstrator's intentions and allowing generalization to states not visited during the demonstration~\cite{brown2019extrapolating}.
%
%However, IRL often requires more sophisticated algorithms and significantly more data or self-supervised experience than BC to reliably infer the underlying reward function. 
%
%Our approach in \algname{} is more aligned with the BC setup where a quick and relatively accurate mimicry of expert behavior is needed without diving deep into the underlying motivations aiming at enhancing the expert performance or transferring the learned knowledge to related tasks. 
%
%BC has proven effective in facilitating end-to-end supervised learning for autonomous robots operating in cluttered and complex environments, such as forest trails~\cite{giusti2015machine} or parking lots and unpaved roads~\cite{bojarski2016end}. There also works that draw insight from both BC and IRL, for instance, Generative Adversarial Imitation Learning (GAIL)~\cite{gail} is an imitation learning method in which a policy network and a discriminator network are jointly trained through an adversarial process.






Some recent works have addressed this issue through generative adversarial training~\cite{goodfellow2014generative}.
%
For instance, Generative Adversarial Imitation Learning (GAIL)~\cite{gail} is an imitation learning method in which a policy network and a discriminator network are jointly trained through an adversarial process. This approach has shown a higher generalizability capacity than traditional IL methods. While GAIL eliminates the need to handcraft a reward function or explicitly compute one from demonstrations, it retains the main shortcomings of deep IL methods: namely, the requirement for large data sets, lack of interpretability, and difficulty in modifying the learned policy. In contrast, \algname\ synthesizes a probabilistic program as the agent's policy from only a dozen of demonstrations. As discussed in the paper, these learned policies are highly interpretable and can be manually refined and improved, which is a specially useful property for closing the simulation-to-real gap in  robotics~\cite{ldips, chebotar2019closing}.  



\paragraph*{Interpretable Learning}



\paragraph*{Probabilistic Program Synthesis}



\section{Related Work (lengthy)} 
 \blue{This is the original text from my literature review. It is currently being summarized in section V}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning and Reward Structures}
Many existing learning frameworks for sequential decision-making employ an explicit reward mechanism.
%
Most notably, Reinforcement Learning (RL) techniques~\cite{sutton2018reinforcement} have been highly successful in solving numerous complex tasks, including playing board games~\cite{silver2017mastering}, video games~\cite{vinyals2019grandmaster}, and performing robotic manipulations~\cite{akkaya2019solving}. These techniques crucially depend on the availability of a reward function or an online discriminator to rank the optimality of candidate policy trajectories~\cite{ross2011reduction}.
%
However, even for experts, it can be challenging to devise reward objectives that lead to desired agent behaviors in complex domains~\cite{boularias2011relative}.
%
Imitation Learning (IL)~\cite{9927439} approaches address this challenge by attempting to learn the desired policy without requiring a reward structure as input.
%
Popular IL methods include Behavioral Cloning (BC)~\cite{ross2011reduction, daftry2017learning, bojarski2016end, giusti2015machine, pomerleau1991efficient}, which aims to learn a function that directly maps observations to actions, and Inverse Reinforcement Learning (IRL)~\cite{ng2000algorithms,ziebart2008maximum,abbeel2004apprenticeship}. IRL seeks to infer the intrinsic reward structure underlying the provided trajectories, modeling the demonstrator's intentions and allowing generalization to states not visited during the demonstration~\cite{brown2019extrapolating}.
%
%
However, IRL often requires more sophisticated algorithms and significantly more data or self-supervised experience than BC to reliably infer the underlying reward function. 
%
Our approach in \algname{} is more aligned with the BC setup where a quick and relatively accurate mimicry of expert behavior is needed without diving deep into the underlying motivations aiming at enhancing the expert performance or transferring the learned knowledge to related tasks. 
%
BC has proven effective in facilitating end-to-end supervised learning for autonomous robots operating in cluttered and complex environments, such as forest trails~\cite{giusti2015machine} or parking lots and unpaved roads~\cite{bojarski2016end}.
%
However, without substantial human feedback and correction, existing BC methods are known to exhibit poor generalization capacity due to compounding errors resulting in distributional shift~\cite{ross2011reduction,tu2022sample}. 
%
Some recent works have addressed this issue through generative adversarial training~\cite{goodfellow2014generative}.
%
For instance, Generative Adversarial Imitation Learning (GAIL)~\cite{gail} is an imitation learning method in which a policy network and a discriminator network are jointly trained through an adversarial process. This approach has shown a higher generalizability capacity than traditional IL methods. While GAIL eliminates the need to handcraft a reward function or explicitly compute one from demonstrations, it retains the main shortcomings of deep IL methods: namely, the requirement for large data sets, lack of interpretability, and difficulty in modifying the learned policy. In contrast, \algname\ synthesizes a probabilistic program as the agent's policy from only a dozen of demonstrations. As discussed in the paper, these learned policies are highly interpretable and can be manually refined and improved, which is a specially useful property for closing the simulation-to-real gap in  robotics~\cite{ldips, chebotar2019closing}.  







\subsection{Learning and Action Labels} 
The problem of learning a policy from trajectories of state-action pairs is referred to as Learning from Demonstrations (LfD). 
%
Most existing agent learning approaches, including RL, IRL, and BC methods, assume the existence of the agent's action labels in the data, and thus target the LfD problem~\cite{daftry2017learning, bain1995framework, bojarski2016end,finn2016guided, gail, ho2016model, ng2000algorithms}.
%
However, the requirement for action labels in the data is a significant limitation. It precludes the use of vast amounts of demonstration data, such as vehicle driving data, which is available in abundance but lacks internal action labels~\cite{maddern20171,cordts2016cityscapes,yu2017baidu}. As a result, there has been a recent shift towards a more challenging setting, Learning from Observations (LfO), where the internal actions taken by the demonstrator remain unknown~\cite{torabi2019recent, ijspeert2002movement, xu2022robot, qin2023learning}. LfO offers a more naturalistic form of learning, closely resembling human imitation~\cite{10064325}. In \algname{}, we introduce a novel solution to the LfO problem.
%

There are several  studies that enhance existing imitation and reinforcement learning algorithms to tackle the LfO problem. For example, \cite{torabi2018behavioral} introduces the Behavior Cloning from Observation (BCO) technique, that addresses the limitation of BC concerning action labels and proposes a new imitation learning algorithm that uses state-trajectory-only data.
In BCO, a task-independent inverse dynamics model of the environment is learned during an exploratory phase, which is then used to infer the missing action labels and train the target policy using behavior cloning. 
%
In \algname{}, we also learn a policy directly from state-trajectory-only data; however, there are significant differences compared to BCO. First, our approach learns policies as probabilistic programs, which allow for interpretation and repair, in contrast to the deep neural policies learned by BCO. 
 %
Additionally, neural approaches, such as BCO, are not sample efficient and require orders of magnitude more data than \algname\ to learn the desired policy. Moreover, BCO necessitates numerous interactions with the environment to understand the inverse dynamic model, whereas our approach is entirely offline, eliminating the need for any post-demonstration interactions with the environment. Instead, \algname{} employs a motion model as its primary input, concentrating on the agent's internal mechanics and dynamics, which is frequently more accessible than a model of the environment~\cite{spong2005robot}.
%
The idea of inferring inverse dynamics models through self-supervised exploration for enhancing and annotating state-only trajectories, has also been explored in the context of manipulating deformable objects~\cite{nair2017combining, pathak2018zero}. However, in these studies, the objective is to learn how to achieve a singular, human-provided target shape, which is a distinct problem from learning a policy for sequential decision making. 


\algname{} is also related to recently enhanced IRL techniques addressing the LfO problem~\cite{torabi2018generative, henderson2018optiongan, liu2018imitation}. For example, GAIfO~\cite{torabi2018generative} is an LfO solution grounded in the GAIL~\cite{gail} framework. It presents a universal framework for imitation from observation without the need for action information. GAIfO has demonstrated the ability to identify imitation policies that perform nearly as well as those developed by techniques with access to action labels.
%
Similarly, OptionGAN~\cite{henderson2018optiongan} extends GAIL to jointly learn the reward and divisions within the demonstration state space simultaneously, thus acquiring the policy and reward options. This facilitates one-shot transfer from noisy demonstrations across different experts and environmental dynamics. 
%
While these methods can learn policies from state-only trajectories, they still require online reinforcement signals during learning, a significant limitation that impacts their usability. Furthermore, IRL methods based on Generalized Adversarial Networks (GAN)~\cite{goodfellow2014generative}, such as GAIfO and OptionGAN, are notoriously challenging to train and scale~\cite{tucker2018inverse}. In contrast, our experimental evaluations show that \algname{} can learn the desired policy with a limited number of trajectories in a relatively straightforward manner.
    
    
    Lastly, there are learning algorithms that employ action labels in a hybrid manner. For instance, the DAgger approach~\cite{ross2011reduction}, which addresses the problem of distributional shift in imitation learning, does not necessitate action labels stored in the data but requires online access to the expert’s labeling during learning. In contrast, \algname{} neither demands online labeling during learning nor within the sequential data.

    










\subsection{Online or Offline Learning}
A fundamental distinction between learning frameworks for sequential decision-making is whether they are online or offline~\cite{prudencio2023survey}. In the online setting, the agent is able to execute candidate policies on the environment during learning, whereas in the offline setting no environment interactions is permitted after the data is collected. 
%
Offline learning is generally more desirable because  execution of intermediate policies in simulation or real world is slow, costly and even dangerous~\cite{chan2021scalable}. Moreover, offline learning enables extensive use and re-use of historical data sets thereby expanding the real-world applicability of the learning approach. 
%
The \algname\ algorithm is an offline approach, and in this part we compare it to existing offline RL, IL and IRL solutions.

While traditional RL algorithms provide a fundamentally online learning
paradigm~\cite{doi:10.1177/0278364913495721, sutton2018reinforcement}, there has been increased recent effort to introduce offline variants of well-known RL techniques to resolve this serious obstacle to their widespread adoption~\cite{konyushkova2020semi, rafailov2021offline, levine2020offline, zolna2020offline, wang2020critic, NEURIPS2022_3908cadf}.
%
Offline reinforcement learning methods (also called Batch RL methods~\cite{lange2012batch}) have been shown to be effective in extracting the desired policy with maximum possible utility from static data-sets of the form $\{(s_t, a_t,r_{t+1},s_{t+1})\}$ that  adequately cover the space of high-reward transitions. However, such reward and action annotations are often unobtainable or highly sparse, e.g. in massive offline data sets of autonomous driving~\cite{caesar2020nuscenes}.  Moreover, practicality of RL-based methods is often limited due to training instability and the compounding of extrapolation errors, and these methods consistently require meticulous hyperparameter tuning through online evaluation. As a result,  pure offline RL methods are seldom used and hybrid approaches that combine offline learning with online exploration have been more successful~\cite{lange2012batch, nair2018overcoming, rajeswaran2017learning, vecerik2017leveraging, pohlen2018observe}. 


In contrast to offline RL methods, the fully offline approach in \algname\ does not require reward signals in the provided trajectories, hence, is more closely related to the works done under offline imitation learning methodologies~\cite{zolna2020offline, liu2021curriculum, jiang2020offline, jarboui2021offline, zeng2023understanding, ross2011reduction}. 
%
%
For instance, ORIL (Offline Reinforced Imitation Learning)~\cite{zolna2020offline} is a recent approach that adopts the GAIL~\cite{gail} framework to the offline setting, and develops an agent that can be trained offline from previously logged robot experiences and a set of expert demonstrations. ORIL first learns a reward model by contrasting the expert demonstrations and logged experiences.  This model is then used to annotate the given trajectories with reward signals, and a policy is learned via offline RL. While ORIL alleviates the need for reward signals in the data-set, it still requires action labels (targets the LfD problem rather than LfO), and also demands hundreds of expert demonstrations and thousands of logged experiences to train a deep neural policy. In contrast, \algname\ only requires a small number of trajectories without any action labels, and synthesizes an interpretable probabilistic program as the agent's policy. 
%
Similarly, AIRL~\cite{fu2017learning} and DemoDICE~\cite{kim2022demodice} are also two recent offline IL methods which learn a policy by first inferring reward structures by comparing exploratory vs expert trajectories in a fully offline way and then using it to disentangle the goals of the expert from the dynamics of the environment, by casting the reward learning problem as a maximum likelihood problem, connecting IRL to generative model training. However, both AIRL and DemoDICE take as input state-action trajectories and require a large number of logged experiences to achieve stability. \blue{todo: clarify better the differences between oril, airl, and demodice} 


Finally, SMODICE~\cite{ma2022versatile} is a recent approach that proposes a versatile algorithm for offline ILfO (imitation learning from observations). Unlike the works mentioned above, learns a policy from state-only-trajectories. Additionally, SMODICE also handles  observations from mismatched experts and environment dynamics, which is a closely related problem However, similar to all deep neural methods mentioned earlier, SMODICE requires a massive number of input data (aroud 200 expert trajectories and 1M logged transitions).










\subsection{Interpretable Learning} 
\begin{itemize}
    \item InfoGAIL~\cite{li2017infogail}: The
goal of this paper is to develop an imitation learning framework that is able to automatically discover
and disentangle the latent factors of variation underlying expert demonstrations. This approach is an extension of GAIL. Similar to InfoGAN's idea, in this paper the mutual information between latent space and trajectories is maximized, resulting in a policy where
low-level actions can be controlled through more abstract, high-level latent variables. This results in an end-to-end imitation learning approach which is able to disentangle different policies used to generate input trajectories. The technique is applied in a self-driving domain where the input is raw pixels and output is continues actions for steering, braking and accelerating. 

\item Programmatically Interpretable Reinforcement Learning (PIRL)
\begin{itemize}
\item \cite{orfanos2023synthesizing} Introduces a connection between ReLU neural networks and oblique decision trees to translate the policy learned with actor-critic algorithms into programmatic policies
\item \cite{koul2018learning} introduces a new technique, Quantized Bottleneck Insertion, to learn finite representations of continuous-valued memory vectors and features in RNN policies trained via RL or IL. The language used is more expressive than if-then-else-only programs and contains loops. 
\item \cite{inala2019synthesizing} proposes an algorithm for learning programmatic state machine policies that can capture repeating behaviors. By doing so, the learned policies have the ability to generalize to instances requiring an arbitrary number of repetitions, a property dubbed inductive generalization. 
\item Programmatic policies in RL and IL can also be obtained with gradient descent and soft decision trees. For instance, \cite{silva2019optimization} uses policy-gradient learning over differentiable decision trees, \cite{ding2020cdt} apply representation learning on the decision path to express policies as Cascading Decision Trees, and \cite{qiu2021programmatic} presents a differentiable program architecture search framework to synthesize interpretable, generalizable, and compositional programs for controlling reinforcement learning applications.
%
%
\item \cite{verma2018programmatically} introduces NDPS, which uses program synthesis to synthesize a “sketch” of a policy and then uses Bayesian optimization to find suitable real-valued parameters for the sketch such that the resulting programmatic policy is as similar as possible to the oracle
\item \cite{verma2019imitation} introduces PROPEL, which trains a neural policy concurrently with the synthesis process to ensure that the neural policy is not “too different” from the programs being synthesized, so it can be more effective in guiding the programmatic search
\item \cite{bastani2018verifiable} proposes VIPER, an algorithm that combines ideas from model compression and imitation learning to learn decision tree policies guided by a DNN policy (called the oracle) and its Q-function.
\end{itemize}
\end{itemize}








\begin{comment}
    \section{Related Work (lengthy)} 
 \blue{This is the original text from literature review. It is being summarized in section V}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning and Reward Structures}
Many existing learning frameworks for sequential decision-making employ an explicit reward mechanism.
%
Most notably, Reinforcement Learning (RL) techniques~\cite{sutton2018reinforcement} have been highly successful in solving numerous complex tasks, including playing board games~\cite{silver2017mastering}, video games~\cite{vinyals2019grandmaster}, and performing robotic manipulations~\cite{akkaya2019solving}. These techniques crucially depend on the availability of a reward function or an online discriminator to rank the optimality of candidate policy trajectories~\cite{ross2011reduction}.
%
However, even for experts, it can be challenging to devise reward objectives that lead to desired agent behaviors in complex domains~\cite{boularias2011relative}.
%
Imitation Learning (IL)~\cite{9927439} approaches address this challenge by attempting to learn the desired policy without requiring a reward structure as input.
%
Popular IL methods include Behavioral Cloning (BC)~\cite{ross2011reduction, daftry2017learning, bojarski2016end, giusti2015machine, pomerleau1991efficient}, which aims to learn a function that directly maps observations to actions, and Inverse Reinforcement Learning (IRL)~\cite{ng2000algorithms,ziebart2008maximum,abbeel2004apprenticeship}. IRL seeks to infer the intrinsic reward structure underlying the provided trajectories, modeling the demonstrator's intentions and allowing generalization to states not visited during the demonstration~\cite{brown2019extrapolating}.
%
%
IRL often requires more sophisticated algorithms and significantly more data or self-supervised experience than BC to reliably infer the underlying reward function. Our approach in \algname{} is more aligned with the BC setup where a quick and relatively accurate mimicry of expert behavior is needed without diving deep into the underlying motivations aiming at enhancing the expert performance or transferring the learned knowledge to related tasks. 
%
BC has proven effective in facilitating end-to-end supervised learning for autonomous robots operating in cluttered and complex environments, such as forest trails~\cite{giusti2015machine} or parking lots and unpaved roads~\cite{bojarski2016end}.
%
However, without substantial human feedback and correction, existing BC methods are known to exhibit poor generalization capacity due to compounding errors resulting in distributional shift~\cite{ross2011reduction,tu2022sample}. 
%
Some recent works have addressed this issue through generative adversarial training~\cite{goodfellow2014generative}.
%
For instance, Generative Adversarial Imitation Learning (GAIL)~\cite{gail} is an imitation learning method in which a policy network and a discriminator network are jointly trained through an adversarial process. This approach has shown a higher generalizability capacity than traditional IL methods. While GAIL eliminates the need to handcraft a reward function or explicitly compute one from demonstrations, it retains the main shortcomings of deep IL methods: namely, the requirement for large data sets, lack of interpretability, and difficulty in modifying the learned policy. In contrast, \algname\ synthesizes a probabilistic program as the agent's policy from only a dozen of demonstrations. As discussed in the paper, these learned policies are highly interpretable and can be manually refined and improved, which is a specially useful property for closing the simulation-to-real gap in  robotics~\cite{ldips, chebotar2019closing}.  







\subsection{Learning and Action Labels} 
The problem of learning a policy from trajectories of state-action pairs is referred to as Learning from Demonstrations (LfD). 
%
Most existing agent learning approaches, including RL, IRL, and BC methods, assume the existence of the agent's action labels in the data, and thus target the LfD problem~\cite{daftry2017learning, bain1995framework, bojarski2016end,finn2016guided, gail, ho2016model, ng2000algorithms}.
%
However, the requirement for action labels in the data is a significant limitation. It precludes the use of vast amounts of demonstration data, such as vehicle driving data, which is available in abundance but lacks internal action labels~\cite{maddern20171,cordts2016cityscapes,yu2017baidu}. As a result, there has been a recent shift towards a more challenging setting, Learning from Observations (LfO), where the internal actions taken by the demonstrator remain unknown~\cite{torabi2019recent, ijspeert2002movement, xu2022robot, qin2023learning}. LfO offers a more naturalistic form of learning, closely resembling human imitation~\cite{10064325}. In \algname{}, we introduce a novel solution to the LfO problem.
%

There are several  studies that enhance existing imitation and reinforcement learning algorithms to tackle the LfO problem. For example, \cite{torabi2018behavioral} introduces the Behavior Cloning from Observation (BCO) technique, that addresses the limitation of BC concerning action labels and proposes a new imitation learning algorithm that uses state-trajectory-only data.
In BCO, a task-independent inverse dynamics model of the environment is learned during an exploratory phase, which is then used to infer the missing action labels and train the target policy using behavior cloning. 
%
In \algname{}, we also learn a policy directly from state-trajectory-only data; however, there are significant differences compared to BCO. First, our approach learns policies as probabilistic programs, which allow for interpretation and repair, in contrast to the deep neural policies learned by BCO. 
 %
Additionally, neural approaches, such as BCO, are not sample efficient and require orders of magnitude more data than \algname\ to learn the desired policy. Moreover, BCO necessitates numerous interactions with the environment to understand the inverse dynamic model, whereas our approach is entirely offline, eliminating the need for any post-demonstration interactions with the environment. Instead, \algname{} employs a motion model as its primary input, concentrating on the agent's internal mechanics and dynamics, which is frequently more accessible than a model of the environment~\cite{spong2005robot}.
%
The idea of inferring inverse dynamics models through self-supervised exploration for enhancing and annotating state-only trajectories, has also been explored in the context of manipulating deformable objects~\cite{nair2017combining, pathak2018zero}. However, in these studies, the objective is to learn how to achieve a singular, human-provided target shape, which is a distinct problem from learning a policy for sequential decision making. 


\algname{} is also related to recently enhanced IRL techniques addressing the LfO problem~\cite{torabi2018generative, henderson2018optiongan, liu2018imitation}. For example, GAIfO~\cite{torabi2018generative} is an LfO solution grounded in the GAIL~\cite{gail} framework. It presents a universal framework for imitation from observation without the need for action information. GAIfO has demonstrated the ability to identify imitation policies that perform nearly as well as those developed by techniques with access to action labels.
%
Similarly, OptionGAN~\cite{henderson2018optiongan} extends GAIL to jointly learn the reward and divisions within the demonstration state space simultaneously, thus acquiring the policy and reward options. This facilitates one-shot transfer from noisy demonstrations across different experts and environmental dynamics. 
%
While these methods can learn policies from state-only trajectories, they still require online reinforcement signals during learning, a significant limitation that impacts their usability. Furthermore, IRL methods based on Generalized Adversarial Networks (GAN)~\cite{goodfellow2014generative}, such as GAIfO and OptionGAN, are notoriously challenging to train and scale~\cite{tucker2018inverse}. In contrast, our experimental evaluations show that \algname{} can learn the desired policy with a limited number of trajectories in a relatively straightforward manner.
    
    
    Lastly, there are learning algorithms that employ action labels in a hybrid manner. For instance, the DAgger approach~\cite{ross2011reduction}, which addresses the problem of distributional shift in imitation learning, does not necessitate action labels stored in the data but requires online access to the expert’s labeling during learning. In contrast, \algname{} neither demands online labeling during learning nor within the sequential data.

    










\subsection{Online or Offline Learning}
A fundamental distinction between learning frameworks for sequential decision-making is whether they are online or offline~\cite{prudencio2023survey}. In the online setting, the agent is able to execute candidate policies on the environment during learning, whereas in the offline setting no environment interactions is permitted after the data is collected. 
%
Offline learning is generally more desirable because  execution of intermediate policies in simulation or real world is slow, costly and even dangerous~\cite{chan2021scalable}. Moreover, offline learning enables extensive use and re-use of historical data sets thereby expanding the real-world applicability of the learning approach. 
%
The \algname\ algorithm is an offline approach, and in this part we compare it to existing offline RL, IL and IRL solutions.

While traditional RL algorithms provide a fundamentally online learning
paradigm~\cite{doi:10.1177/0278364913495721, sutton2018reinforcement}, there has been increased recent effort to introduce offline variants of well-known RL techniques to resolve this serious obstacle to their widespread adoption~\cite{konyushkova2020semi, rafailov2021offline, levine2020offline, zolna2020offline, wang2020critic, NEURIPS2022_3908cadf}.
%
Offline reinforcement learning methods (also called Batch RL methods~\cite{lange2012batch}) have been shown to be effective in extracting the desired policy with maximum possible utility from static data-sets of the form $\{(s_t, a_t,r_{t+1},s_{t+1})\}$ that  adequately cover the space of high-reward transitions. However, such reward and action annotations are often unobtainable or highly sparse, e.g. in massive offline data sets of autonomous driving~\cite{caesar2020nuscenes}.  Moreover, practicality of RL-based methods is often limited due to training instability and the compounding of extrapolation errors, and these methods consistently require meticulous hyperparameter tuning through online evaluation. As a result,  pure offline RL methods are seldom used and hybrid approaches that combine offline learning with online exploration have been more successful~\cite{lange2012batch, nair2018overcoming, rajeswaran2017learning, vecerik2017leveraging, pohlen2018observe}. 






In contrast to offline RL methods, the fully offline approach in \algname\ does not require reward signals in the provided trajectories, hence, is more closely related to the works done under offline imitation learning methodologies~\cite{zolna2020offline, liu2021curriculum, jiang2020offline, jarboui2021offline, zeng2023understanding, ross2011reduction}. 
%
%
%
%
%
For instance, ORIL (Offline Reinforced Imitation Learning)~\cite{zolna2020offline} is a recent approach that adopts the GAIL~\cite{gail} framework to the offline setting, and develops an agent that can be trained offline from previously logged robot experiences and a set of expert demonstrations. ORIL first learns a reward model by contrasting the expert demonstrations and logged experiences.  This model is then used to annotate the given trajectories with reward signals, and a policy is learned via offline RL. While ORIL alleviates the need for reward signals in the data-set, it still requires action labels (targets the LfD problem rather than LfO), and also demands hundreds of expert demonstrations and thousands of logged experiences to train a deep neural policy. In contrast, \algname\ only requires a small number of trajectories without any action labels, and synthesizes an interpretable probabilistic program as the agent's policy. 
%
Similarly, AIRL~\cite{fu2017learning} and DemoDICE~\cite{kim2022demodice} are also two recent offline IL methods which learn a policy by first inferring reward structures by comparing exploratory vs expert trajectories in a fully offline way and then using it to disentangle the goals of the expert from the dynamics of the environment, by casting the reward learning problem as a maximum likelihood problem, connecting IRL to generative model training. However, both AIRL and DemoDICE take as input state-action trajectories and require a large number of logged experiences to achieve stability. \blue{todo: clarify better the differences between oril, airl, and demodice} 


Finally, SMODICE~\cite{ma2022versatile} is a recent approach that proposes a versatile algorithm for offline ILfO (imitation learning from observations). Unlike the works mentioned above, learns a policy from state-only-trajectories. Additionally, SMODICE also handles  observations from mismatched experts and environment dynamics, which is a closely related problem However, similar to all deep neural methods mentioned earlier, SMODICE requires a massive number of input data (aroud 200 expert trajectories and 1M logged transitions). \blue{dig deeper and figure out more fundamental differences}.










\subsection{Interpretable Learning} 
\begin{itemize}
    \item InfoGAIL~\cite{li2017infogail}: The
goal of this paper is to develop an imitation learning framework that is able to automatically discover
and disentangle the latent factors of variation underlying expert demonstrations. This approach is an extension of GAIL. Similar to InfoGAN's idea, in this paper the mutual information between latent space and trajectories is maximized, resulting in a policy where
low-level actions can be controlled through more abstract, high-level latent variables. This results in an end-to-end imitation learning approach which is able to disentangle different policies used to generate input trajectories. The technique is applied in a self-driving domain where the input is raw pixels and output is continues actions for steering, braking and accelerating. 

\item Programmatically Interpretable Reinforcement Learning (PIRL)
\begin{itemize}
\item \cite{orfanos2023synthesizing} Introduces a connection between ReLU neural networks and oblique decision trees to translate the policy learned with actor-critic algorithms into programmatic policies
\item \cite{koul2018learning} introduces a new technique, Quantized Bottleneck Insertion, to learn finite representations of continuous-valued memory vectors and features in RNN policies trained via RL or IL. The language used is more expressive than if-then-else-only programs and contains loops. 
\item \cite{inala2019synthesizing} proposes an algorithm for learning programmatic state machine policies that can capture repeating behaviors. By doing so, the learned policies have the ability to generalize to instances requiring an arbitrary number of repetitions, a property dubbed inductive generalization. 
\item Programmatic policies in RL and IL can also be obtained with gradient descent and soft decision trees. For instance, \cite{silva2019optimization} uses policy-gradient learning over differentiable decision trees, \cite{ding2020cdt} apply representation learning on the decision path to express policies as Cascading Decision Trees, and \cite{qiu2021programmatic} presents a differentiable program architecture search framework to synthesize interpretable, generalizable, and compositional programs for controlling reinforcement learning applications.
%
%
\item \cite{verma2018programmatically} introduces NDPS, which uses program synthesis to synthesize a “sketch” of a policy and then uses Bayesian optimization to find suitable real-valued parameters for the sketch such that the resulting programmatic policy is as similar as possible to the oracle
\item \cite{verma2019imitation} introduces PROPEL, which trains a neural policy concurrently with the synthesis process to ensure that the neural policy is not “too different” from the programs being synthesized, so it can be more effective in guiding the programmatic search
\item \cite{bastani2018verifiable} proposes VIPER, an algorithm that combines ideas from model compression and imitation learning to learn decision tree policies guided by a DNN policy (called the oracle) and its Q-function.
\end{itemize}
\end{itemize}
\end{comment}







%\subsection{Learning from Noisy Data}
%Here categorize various forms of noise that can manifest in sequential data and discuss why probabilistic programs are a suitable formalism to generalize noisy trajectories into a policy.  \blue{todo}



\begin{comment}
\paragraph{Expectation-Maximization Techniques}

The expectation maximization algorithm is a commonly used technique in scenarios where the generative model and its hidden states are both unknown~\cite{em}. EM has found some recent applications in various robotics domains. For instance, in \cite{steady}, the authors propose to use an EM loop to learn a dynamics model and estimate the robot's state trajectories simultaneously. In \cite{Inala2020Synthesizing}, an internal expectation-maximization loop was used to optimize the learned policy, but this approach focuses on reinforcement learning applications and is not suitable for handling high levels of noise. In contrast, our approach utilizes an EM loop to infer labels from noisy demonstrations while synthesizing a complex probabilistic program that maximizes the demonstration likelihood.


\paragraph{Probabilistic Program Synthesis}
The goal of probabilistic program synthesis is to obtain a probabilistic program from partial observations, which can then be leveraged for statistical inference or sampling purposes \cite{10.1145/3290350}. Prior work has used Markov Chain Monte Carlo (MCMC) methods to generate distributions over programs \cite{10.1145/3290350,10.1145/3140587.3062375}. However, our work uses an alternative technique based on a combination of enumerative synthesis and numerical optimization. Our approach can be seen as a generalization of earlier deterministic policy synthesis methods such as \cite{ldips}, which uses an SMT solver to maximize the number of satisfied examples. Additionally, the probabilistic program we develop incorporates ``logistic thresholds" to capture uncertainties in natural phenomena, an idea that was recently explored in~\cite{qiu2022programmatic}.
\blue{TODO: menion LLMs and why they are not a good fit for such synthesis tasks. }

% alternative technique for synthesizing deterministic state-machine policies that is better suited to our problem. By separating each transition, we have simplified the problem, making it amenable to enumeration and optimization. 

\end{comment}

%%%% OLD RW
%\paragraph{Learning from Expert Demonstrations} The problem addressed in this paper is related to a major challenge in machine learning, which is to learn a policy by observing expert demonstrations without explicit reinforcement signals~\cite{https://doi.org/10.48550/arxiv.2102.12667,https://doi.org/10.48550/arxiv.1910.13395}. 
%
%Various solutions have been proposed, generally separated into two categories. \textit{Behavioral cloning} learns a classifier by performing supervised learning over state-action pairs~\cite{10.5555/3304652.3304697}. \textit{Inverse reinforcement learning} applies reinforcement learning techniques after learning an unspecified reward function~\cite{10.5555/3045390.3045397,ziebart2008maximum}.
%
%Both approaches have been successfully used to solve complex tasks, such as object manipulation or surgery~\cite{doi:10.1177/0278364914554471,DBLP:journals/corr/RahmatizadehABL17}.
%
%In particular, \textit{Generative Adversarial Imitation Learning} (GAIL)~\cite{gail}
%is a popular technique for imitation learning that attempts to match the occupancy measure of the expert.  
%Extensions to these techniques have been developed to handle environment noise~\cite{https://doi.org/10.48550/arxiv.1804.02477}.
% Unlike IRL techniques, which rely on the ability to interact with the environment and collect additional data, \algname{} does not require interacting with the environment and only requires a motion model, which is more readily available.
%Second, our approach utilizes \textit{low-level controllers} to more accurately predict low-level outputs. 
%As our experiments demonstrate, the ability to utilize user-provided motor controllers greatly improves performance in settings with high noise. Program synthesis over high-level controllers is explored in~\cite{https://doi.org/10.48550/arxiv.1804.02477}, but this work is restricted to a reinforcement learning setting.
%
%Additionally, techniques that involve neural networks tend to be data-intensive, non-interpretable, and not amenable to repair~\cite{2018arXiv180406557S}. To the best of our knowledge, our approach is the first to synthesize a symbolic policy from noisy and unlabeled demonstrations.
%







%We attempted to use GAIL to generate a neural policy to imitate trajectories, but this approach yielded results with abysmal log-likelihood scores. However, the shape generated by these policies still resembled the ACC-CON-DEC pattern embedded in the data. We believe that GAIL's failure to perform well on this task is due to its goal (matching an expert's occupancy measure) being inherently different than the other baselines; for GAIL the correctness of each individual low-level action matters less than the trajectory as a whole.


==> res_fig.tex <==
% example figures
\begin{figure*}[t]
\centering
\begin{subfigure}[t]{0.42\textwidth}
\centering
%\hspace*{-0.5cm} 
    \includegraphics[width=1\textwidth]{figs/1D-target-emloop.png}
    \caption{Progress of EM loop until convergence in the \textit{Target} benchmark. 
    %Results for the testing set are similar to that of the training set, indicating that our approach generalizes well.
    }
    \label{fig:loop_progress}
\end{subfigure}
\qquad
\begin{subfigure}[t]{0.42\textwidth}
\centering
%\hspace*{-0.5cm} 
    \includegraphics[width=\textwidth]{figs/noise.png}
     \caption{Accuracy of baselines
     %relative to the ground truth policy, 
     at varying levels of noise in \textit{Merge} benchmark.
     %Experiments are performed on the . 
     %Noise levels are scaled to fit the range $[0, 1]$ for presentation purposes.
     }
    \label{fig:noise}
\end{subfigure}
%\hfill
%\begin{subfigure}[t]{0.32\textwidth}
%\centering
%\hspace*{-0.5cm} 
%    \includegraphics[width=1.13\textwidth]{figs/ldips.png}
%    \caption{Progress of EM loop using deterministic vs. probabilistic synthesis}
%    \label{fig:ldips}
%\end{subfigure}
\caption{Experimental Results}
\label{fig:demos}
\end{figure*}


==> sec3.tex <==
\begin{comment}
    3) The EM Synthesis Algorithm:
- math for EM (what math objective it's optimization and why it works --> markovian system motivates ASP structure)
- E step (particle filter)
    - observation likelihood calculations (including multi-dimensional LAs)
- more details in the M step. (how we combine symbolic search with numerical optimization) 
    - splitting into transitions between labels
    - numerical optimization details, including how we handle ANDs and ORs
    - Describe the incremental program synthesis technique where we enumerate over programs that are similar to the current program - this involves manipulating both features and clauses
        - citation for principle that syntactically similar programs are often semantically similar?
- Any other interesting tricks we did + any hyperparameters
    - program complexity, "alpha loss" flattening (unclear how much the latter does)
    - use of LDIPS framework -> dimension-informed in addition to standard program synthesis benefits like observational equivalence
    - start with heuristic labeler that prefers maintaining the same state
\end{comment}

%\renewcommand{\theequation}{\Roman{equation}}
\section{Problem Formulation  (old -- this is being rewritten)}
%In this section, we present  a comprehensive overview of the \algname{} algorithm.

%\subsection{Algorithm Overview} 
%\label{sec:formulation}

We aim to infer a \emph{maximum a posteriori (MAP)} estimate of a probabilistic ASP, $\asp^*$, using only human demonstrations of low-level action trajectories, $l_{1:t}$ (e.g., the steering and accelerator control signals), and the corresponding robot states, $s_{1:t}$ (e.g., the velocity of the vehicle), i.e., 
%
\begin{equation} \small
    \asp^* = \argmax\limits_{\asp} P(l_{1:t}|s_{1:t}, \asp) P(\asp) \label{eq:problem_statement}
\end{equation}
%
where $P(\asp)$ specifies the prior probability (density) of ASPs. Note that the ASPs can contain unknown parameters, whose distribution is also specified in this prior.
%
We next introduce high-level action labels, $h_{1:t}$, as latent variables which can be marginalized out as follows: 
\begin{equation} \small
   \asp^* = \argmax_{\asp} \sum_{h_{1:t}} P(l_{1:t} | h_{1:t}, s_{1:t}) P(h_{1:t}|s_{1:t}, \asp) P(\asp)\ \label{eq:map-objective}
\end{equation}
where $P(l_{1:t} | h_{1:t}, s_{1:t})$ is the motion model that defines the likelihood of the low-level actions given the high-level action labels and the robot states, and $P(h_{1:t}|s_{1:t}, \asp)$ is the label sequence probability according to the ASP. We also make the Markov assumptions on the ASP and motion model, i.e.,
\vspace{-2mm}
%\begin{equation} \small
%   \asp^* = \argmax_{\asp} \sum_{h_{1:t}}. \prod_{i=1}^t P(l_i|h_i, s_i). \prod_{i=1}^t P(h_i|h_{i-1}, s_i, \asp). P(\asp)\ \label{eq:map-objective}
%\end{equation} 
%\vspace{-2mm}
\begin{equation} \small
    P(h_{1:t}|s_{1:t},\asp) = \prod_{i=1}^t P(h_i|h_{i-1}, s_i, \asp),
    \label{eq:transition-prob}
\end{equation} 
\vspace{-2mm}
\begin{equation} \small
    P(l_{1:t}|h_{1:t},s_{1:t}) = \prod_{i=1}^t P(l_i|h_i, s_i). \ \ \ \ \ 
    \label{eq:motor-model}
\end{equation} 
\vspace{-3mm}

%We further make the Markov assumption that the high-level action labels are conditionally independent given the robot state, the ASP, and the label from the last time step. Hence, we have 

%and similarly, we also assume the motion model is Markovian and have



%High-level action labels, $h_{1:t}$, are unknown, and the optimal MAP estimate $\asp^*$ is the ASP that maximizes the likelihood of the demonstrated actions after marginalizing out the high-level action labels:
%\begin{multline}
%    \asp^* = \argmax_{\asp} P(l_{1:t}|s_{1:t}, \asp) P(\asp) \\[-1mm]
%     = \argmax_{\asp} \sum_{h_{1:t}} P(l_{1:t} | h_{1:t}, s_{1:t}) %P(h_{1:t}|s_{1:t}, \asp) P(\asp)\ \label{eq:map-objective}
%\end{multline}
%where $P(l_{1:t} | h_{1:t}, s_{1:t})$ is the motion model that defines the likelihood of the low-level actions given the high-level action labels and the robot states, $P(h_{1:t}|s_{1:t}, \asp)$ is the label sequence probability according to the ASP, and 

%$P(\asp)$ specifies the prior probability (density) of each ASP (note that the ASP can contain unknown parameters, whose distribution is also specified in this prior).



%The hidden variables in this problem are the high-level action labels $h_{1:t}$ (\eg{} whether to slow down, speed up, or switch lanes), which are unknown. The optimal MAP estimate

%There are two major challenges in solving the above MAP estimate. First, directly computing the sum in \eqref{eq:map-objective} is computationally intractable, and second, the search space of ASPs is huge and involves a searching for a combinatorial structure space while optimizing its parameters in a continuous space.



There are two major challenges in solving the above MAP estimate. First, directly computing the sum in \eqref{eq:map-objective} is computationally intractable. Second, the search space of ASPs is prohibitively large, requiring a combinatorial search through a syntactical space while simultaneously optimizing parameters in a continuous domain.
%
These two challenges motivated us to design a novel Expectation-Maximization (EM) algorithm to approximate and iteratively improve the desired MAP estimate.
%
%Algorithm~\ref{alg:overview} presents a summary of our approach. The algorithm takes as input the low-level demonstrations, the motion model, the initial distribution of action labels, and the initial policy $\pi^{(0)}$. The algorithm then cycles between the E step (lines 2-3) where it performs a posterior sampling using the current ASP, and the M step (line 4) where it synthesizes a policy that is maximally consistent with the sampled trajectories from the E step. 
Algorithm~\ref{alg:overview} presents a summary of our approach. The algorithm takes as input the low-level demonstrations, the motion model, the initial distribution of action labels, and the initial policy $\pi^{(0)}$. 
The algorithm then alternates between the E step (lines 2-3), where it performs posterior sampling using the current ASP, and the M step (line 4), where it synthesizes a policy that is maximally consistent with the sampled trajectories from the E step. Both of the E and M steps are more tractable than solving \eqref{eq:map-objective}, and under certain mild assumptions, the cycle described in Algorithm~\ref{alg:overview} is guaranteed to increase the likelihood of the demonstrations given the synthesized policy~\cite{em,steady}. Thus, the EM cycle can be  repeated until convergence, at which point the desired ASP, $\asp^*$, is identified and returned. In the following we describe the E and M steps of the algorithm in more details. 




 %

 %and returns an optimal ASP $\asp^*$. 
 %
 %To speed up convergence, it is important that $\asp^{(0)}$ is defined in a way that kickstarts the EM loop with a reasonably good initial label sequences. We find that a trivial ASP that randomly switches its label from the last time step with a small probability $p = 0.1$ works well. Intuitively, this corresponds to the idea that human demonstrations are likely to remain in the same high-level label for long periods of time. 
%
%Under certain mild assumptions, the EM cycle described in Algorithm~\ref{alg:overview} is guaranteed to increase the likelihood of the demonstrations, as shown in~\cite{steady,em}. Thus, the cycle can be iteratively repeated until convergence, at which point the desired ASP, $\asp^*$, is identified and returned. In the following we describe the E and M steps of the algorithm in more details. 


 
\paragraph*{E Step}
 At each iteration $k$ in Algorithm~\ref{alg:overview}, the
E step (lines 2-3) uses the current estimate of the ASP $\asp^{(k)}$ to sample $N$ plausible high-level action sequences from the posterior distribution $h^i_{1:t} \sim P(h_{1:t} \mid s_{1:t}, l_{1:t}, \asp^{(k)})$, $i=1\ldots N$. This posterior sampling problem is well-studied in the robotics literature and can be solved using existing state estimation techniques~\cite{thrun2002probabilistic}. 
%
We use a standard particle filter~\cite{doucet2009tutorial} to sample action label sequences.
In particular, the particle filter uses the ASP to sample action labels (the ``particles") forward in time and the motion model to reweight and resample particles such that the ones more consistent with the current observation are more likely to be duplicated. To obtain the full trajectory samples, we take samples from the last time step and trace back in time following the ancestral lineages. 
%





%from the posterior distribution $h^i_{1:t} \sim P(h_{1:t} \mid s_{1:t}, l_{1:t}, \asp^{(k)})$, for $i=1\ldots N$. T

\paragraph*{M Step} During the M Step in Algorithm~\ref{alg:overview} (line 4), a new ASP is synthesized by solving the following equation, where the ASP search space $\mathcal{N}(\asp^{(k)})$ denotes the set of ASPs that are syntactically similar to $\asp^{(k)}$, and the label sequences~$h^i_{1:t}$ are taken from the previous E step: 
\begin{equation} \small \label{eq:optimal-synthesis}
    \asp^{(k+1)} = \argmax_{\asp \in \mathcal{N}(\asp^{(k)})} \log P(\asp) + \frac{1}{N}  \sum_{i=1}^N \log P(h^i_{1:t} \mid s_{1:t},\asp)
\end{equation}
%


To synthesize a policy that is maximally consistent with the trajectories according to \eqref{eq:optimal-synthesis}, we first decompose the trajectories into individual transitions at every time step. These can be used as positive and negative \textit{examples} for the desired transition conditions.
%
For each initial action label $h_1$, we synthesize a probabilistic condition  $\phi_{h_1,h_2}$ for transitions to every other target label $h_2$, using this set of examples.
%
Each $\phi$ is a Boolean expression with \textit{probabilistic thresholds}, as described by the syntax in \autoref{fig:syntax}. These formulas are constructed by enumerating over the set of user-provided numerical expressions, including domain functions, variables, and constants. These numerical expressions serve as \textit{features} for defining the probabilistic thresholds. We then enumerate over conjunctions and disjunctions of these predicates up to a specified depth. 
% 



However, the above method for enumerating programs quickly becomes intractable, especially when the synthesis step is integrated within the EM loop, which might require many iterations to converge. 
%
To address this, we leverage the iterative nature of the EM algorithm and design an incremental synthesis algorithm across M Steps. 
%
We restrict the search space to just the neighborhood of the current best policy, in addition to a set of base predicates that allows the synthesis step to ``reset" to a simple program. 
%
This design is inspired by the success of evolutionary algorithms~\cite{Namdeo2017EvolutionaryAF}. 
%
 To enumerate the neighborhood, we mutate the abstract syntax tree of the current ASP to obtain syntactically similar expressions. 
 %
 These mutations include swapping features and operators, and adding or removing predicates. 
A comprehensive description of all mutations 
%is omitted due to space constraints and 
can be found in the public repository for \algname{}. \blue{( maybe now that we have more space we should list them again)}
%
Moreover, to further prune the search space, we adopt a type system grounded in physical dimensional constraints, as previously done in \cite{ldips}. This type system tracks the physical dimensions of expressions, discarding those that are physically meaningless. 
%

The above two pruning methodologies substantially decrease the program search space, yet still allow for the exploration of increasingly intricate expressions.




%We use the following five types of mutations: 
%\begin{enumerate}
%    \item adding a predicate with a random base feature,
%    \item removing predicates,
%    \item swapping conjunctions and disjunctions,
%    \item augmenting numerical expressions with a random operation and a %random base feature,
%    \item simplifying numerical expressions by removing an operation.
%\end{enumerate}


Finally, each candidate program structure enumerated in the above fashion, must be completed with constants that optimize \eqref{eq:optimal-synthesis}.
In particular, each logistic function used in partial programs contains two unknown constants, $k$, which controls the slope of the logistic curve, and $x_0$, which controls the horizontal offset. 
%
We solve for these parameters using the line search gradient descent (L-BFGS)  algorithm and take the best results from multiple random initial values. 



%ach input example is classified as a \textit{positive} or \textit{negative} example for a given transition. We then optimize for the transition probabilities over all examples using the Markov assumption according to \eqref{eq:transition-prob}. To handle conjunctions, we use the recursive formula $P(e_1 \text{ and } e_2) = P(e_1) \times P(e_2)$, and similarly, for disjunctions we use $P(e_1 \text{ or } e_2) = P(e_1) + P(e_2) - P(e_1 \text{ and } e_2)$, where $P(e)$ denotes the probability of the predicate expression $e$ being true, which is given by the logistic function or calculated using one of the above formulae.




%To prevent the synthesizer from simply adding predicates at each iteration to cover all cases and overfitting to the sampled labels, we define the ASP prior used in \eqref{eq:optimal-synthesis} as $\log P(\asp) = -c_1 \cdot \mathrm{size}(\asp) - c_2 \sum_{k \in \asp} k^2$ (for some constants $c_1, c_2>0$) to penalize large programs (according to the size of their AST) and overconfident conditions.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%Our algorithm, \algname{}, works by alternating between two steps that are each more tractable than \eqref{eq:map-objective}. 

%\algname{} starts by taking in an initial ASP $\asp^{(0)}$, which may be inaccurate but serves as a starting point. 


%Then, at each iteration $k$, the Expectation (E) Step uses the current estimate of the ASP $\asp^{(k)}$ to sample $N$ plausible high-level action sequences from the posterior distribution $h^i_{1:t} \sim P(h_{1:t} \mid s_{1:t}, l_{1:t}, \asp^{(k)})$, $i=1\ldots N$. 






%\subsection{Sampling Posterior Label Sequences (E Step)}
%\label{sec:particle_filter}
%We use a standard particle filter to sample $N$ action label sequences from the posterior distribution $h^i_{1:t} \sim P(h_{1:t} \mid s_{1:t}, l_{1:t}, \asp^{(k)})$, for $i=1\ldots N$. The particle filter uses the ASP to sample action labels (the ``particles") forward in time and the motion model to reweight and resample particles such that the ones more consistent with the current observation are more likely to be duplicated. To obtain the full trajectory samples, we take samples from the last time step and trace back in time following the ancestral lineages.

%To use the particle filter, we alternate between forward sampling via our programmatic prior and resampling. In the forward sampling step, we run our policy on the set of particles from the last time step to obtain a new set of particles following ${h^i_t}_i^M$. In the resampling step, we re-weight each particle based on the low-level action likelihood. Particles that are more consistent with the demonstration are duplicated and replace particles that are less likely. Finally, we generate full trajectories by tracing the ancestral lineage of each particle picked from the last time step. 
%\paragraph{motion model} motion models are user-defined, programmatic controllers designed to perform different tasks specified by the high-level labels. We define our motion model $P(l_t|h_t, s_t)$ as a function from the current action label and state to a distribution over low-level actions. To capture the errors and imperfections of real-world demonstrations, we model the output as a Gaussian distribution centered around the ideal low-level actions output by the controllers. 
% We note that although we assume a Gaussian noise distribution, our implementation is modularized to support easy integration of custom non-Gaussian noise models as well.
%\paragraph{Initial ASP} To speed up convergence, we initialize $\asp^{(0)}$ in a way that kickstarts the EM loop with good initial label sequences. We find that a simple ASP that randomly switches its label from the last time step with a small probability $p = 0.1$ works well. Intuitively, this corresponds to the idea that human demonstrations are likely to remain in the same high-level label for long periods of time.





%In standard deterministic synthesis, these features are then compared to constant holes to form a predicate.  However, in order to provide distributions over transitions in the next E Step, we need to synthesize a probabilistic program.  We do so by representing predicates as logistic functions over expressions, which can be viewed as comparisons with \textit{probabilistic thresholds}. Finally, we enumerate over conjunctions and disjunctions of these predicates, up to a given depth.



%However, this form of enumeration over programs quickly becomes intractable, especially because the synthesis step needs to be embedded inside the EM loop, which may take many iterations to converge. Instead, we take advantage of the iterative nature of the EM algorithm and use incremental synthesis in the M Step.
%note that if a program performs poorly in one iteration, it is unlikely to perform well in subsequent iterations. 


==> sec4.tex <==
\section{Experimental Evaluations (This is Being re-written)}
\label{sec:eval}
In this section, we evaluate our approach by comparing it to baselines in solving five standard imitation learning tasks from two challenging environments.


\subsection{Environments and Tasks}
%We applied \algname{} and the baseline approaches in two challenging domains, autonomous driving and manipulation of a robotic arm.
\noindent \textit{\textbf{Autonomous Vehicle (AV)}}:
We utilized the open-source simulation environment \textsc{highway-env}~\cite{Eleurent2021}, where the demonstrator controls a vehicle moving on a straight highway.
%
We defined the following three tasks within this environment.
%
The Stop Sign (SS) task, is the motivating example described in \autoref{sec:overview} and involves the demonstrator controlling the vehicle's acceleration in order to move to and stop at target locations without changing lanes or any traffic on the road. \jimmy{just to be clear, this isn't implemented in highway-env, though I assume it isnt a big deal}
%
The Pass Traffic (PT) task is more complex and involves ongoing traffic. In this task, the agent's goal is to switch lanes appropriately to pass slower traffic.
%using the high-level actions \textit{accelerate, decelerate, turn left}, and \textit{turn right}. 
 %
 %
Finally, in the Merge (MG) task, the vehicle starts in the left-most lane, and the expected behavior is to merge swiftly into the rightmost lane without colliding with the moving traffic.
 %This scenario uses the same high-level actions as HW. 
% The low-level actions for SS is only the vehicle's \textit{acceleration} value, and for PT and MG isthe amount of \textit{acceleration} and \textit{steering}. 


\noindent \textit{\textbf{Robotic Arm (RA)}}:
We utilized the open-source environment \textsc{panda-gym}~\cite{gallouedec2021pandagym}, which simulates a Franka Emika Panda robotic arm with seven degrees of freedom \jimmy{the 7 degrees of freedom isn't really relevant and potentially misleading, since we only have 4 low-level action dimensions}. We evaluated our approach using two tasks defined in this environment. The first is the Pick and Place (PP) task, which requires the arm to grab an object and then move it to a designated location. The second is the Stack (ST) task, which is more complex and requires stacking two boxes on top of each other in the correct order.


%The first five columns in  \autoref{tab:tasks_demos} present further details about each of the above task, including the number of state variables $|s_i|$, number of high-level action labels, $|h_i|$, and the size of low-level action space, $l_i$. For instance, for the SS task, there are six state variables, $\{\}$, three high-level action labels, $\{\ACC,\DEC,\CON\}$, and a single low-level action, $\{acc\}$.
% The remaining columns in \autoref{tab:tasks_demos} present the details of the demonstrations generated for training and testing the imitation learning tasks. In particular, it shows the average length of the demonstrations and the number of trajectories used for training and testing. 

The first file \jimmy{file?} columns in 
\autoref{tab:tasks_demos} present more details about the above tasks. Specifically, $|s_i|$ is the number of state variables, $|a_i|$ is the number of action labels, and $|z_i|$ is the number of low-level observation variables. 
%
For instance, in the SS task, the state variables are $\{pos, v, v_{max}, a_{min}, a_{max}, d_{stop}\}$, the action labels are $\{\ACC, \DEC, \CON\}$, and the low-level observation is $\{acc\}$.
%
The subsequent columns in \autoref{tab:tasks_demos} detail the demonstrations used for imitation learning, including average trajectory length and the number of trajectories in the training and test sets. A comprehensive description of all tasks and demonstrations can be found in the public repository for \algname{}. \jimmy{I think the trajectory length is probably not relevant, since the size of each timestep is kind of arbitrary}








\subsection{Baselines}
We compare \algname{} against two state-of-the-art IL
approaches and two variations of our algorithm to validate
our design choices.


    \noindent
    \textit{\textbf{FitGreedy}}. This baseline
is a variation of the \algname{}  in which instead of iteratively improving the action label estimates, each time step is labeled greedily with the action label whose likelihood is highest according to the motion model. \blue{what does this show?} \jimmy{This is kiiind of a variation of our algorithm. I prefer the formulation in the previous paper; it shows how this approach is the intuitive solution to the problem but doesn't work well. See below:}

    \noindent
    \textit{\textbf{FitGreedy}}. This baseline represents the intuitive solution to the unlabeled trajectories problem, where each time step is labeled greedily with the action label whose likelihood is highest according to the motion model. Program synthesis is then performed over the acquired labels.

    \noindent
    \textit{\textbf{FitSmooth}}. This baseline is similar to FitGreedy, but it labels trajectories using a particle filter and the $\stx{randSwitch}(0.1)$ ASP. This baseline can be viewed as the first iteration of \algname{}, except that it does not employ incremental synthesis and directly searches over a large program space.

    \noindent
    \textit{\textbf{BC/BC+}}. The BC baseline implements behavior cloning, a well-established IL technique. We trained an LSTM with 64 hidden units to predict the next low-level observation in test trajectories conditioned on all previous states and low-level observations.
    %
    BC+ extends the BC baseline with access to the motion model. Instead of using the LSTM to directly output the low-level observation, we let the neural network output a distribution over all available actions labels and then perform a weighted sum over the corresponding low-level observations, obtained by running the motion model. 
    

    \noindent \textit{\textbf{GAIL}}. This approach is the state-of-the-art IL method for learning a policy directly from expert trajectories. It 
    iterates between training a generator and discriminator neural network, following the approach in Generative Adversarial Networks (GAN)~\cite{goodfellow2014generative}. Our generator consists of \fixme{X} fully connected layers, each one with \fixme{X} neurons; our discriminator is \fixme{X} layers of \fixme{X} neurons each.
    %
Similar to the BC baseline, the {GAIL} baseline directly predicts low-level observations and is not given high-level action labels or the motion model. As a result, the bare-bone version of GAIL shows poor performance for all tasks. \jimmy{hopefully this is no longer the case after new experiments?}

\jimmy{We also note that {GAIL}, like inverse reinforcement learning (IRL) methods, can query the simulation environment during training, while the other algorithms mentioned do not. This limits the applicability of {GAIL} in real-world problems where such access is difficult to obtain.}


%    \textit{\textbf{GAIL}}. This approach is the state-of-the-art imitation learning method for learning a policy directly from expert trajectories. It iterates between training a generator and discriminator neural network in a GAN-like manner, where the generator attempts to minimize discriminator accuracy, and the discriminator tries to maximize its ability to differentiate between expert and generator trajectories. Our generator consists of 3 fully connected layers, each one with 32 neurons; our discriminator is 2 layers of \fixme{?} neurons each. Similar to the \textit{BC} algorithm, \textit{GAIL} is not given high-level action labels or the motion model; however, similar to the RL setting, it can query a simulation with actions to generate its own samples. \fixme{???}




\subsection{Implementation}
\jimmy{what's this for?}

%\newpage


% follosing is a large full page width table containing the acc and log ll results in addition to task and demo descriptions
\begin{comment}
\begin{table*}
\footnotesize
\caption{\label{tab:pct_accuracy} Main Benchmark Results}
\centering

\begin{tabular}{|ccccc|ccc|cccccc|}
    \toprule
    \multicolumn{5}{|c}{\textbf{Tasks}}  &   
    \multicolumn{3}{|c}{\textbf{Demonstrations}}  &  
    \multicolumn{6}{|c|}{\textbf{Accuracy(\%) $/$ Log\,Obs.\,Likelihood}}
        \\
        \tabheader{|c}{ID}                  &   
        \tabheader{c}{Env} & 
        \tabheader{c}{$|s_i|$} &
        \tabheader{c}{$|h_i|$} & 
        \tabheader{c}{$|l_i|$} & 
        \tabheader{|c}{avg.\,len.} & 
        \tabheader{c}{train} & 
        \tabheader{c}{test} &
        \tabheader{|c}{FitGreedy} & 
        \tabheader{c}{FitSmooth} &
        \tabheader{c}{BC} & 
        \tabheader{c}{BC+} &
        \tabheader{c}{GAIL} & 
        \tabheader{c|}{\algname{}} 
        \\
    \midrule
    %
    SS & AV & 6 & 3  & 1 & 125 & 10 & 20 & 60.6$\,/\,$-2.19 & 88.3$\,/\,$-1.12 & NA$\,/\,$-4.60 & 78.0$\,/\,$-1.24 & xx.x$\,/\,$xx.x  & \textbf{98.6$\,/\,$-0.78} \\
    PT & AV & 8 & 4  & 2 & 150 & 10 & 20 & 67.9$\,/\,$-2.10 & 87.1$\,/\,$-0.47 & NA$\,/\,$-1.00 & 70.8$\,/\,$-1.71 & xx.x$\,/\,$xx.x & \textbf{94.7$\,/\,$0.37} \\
    MG & AV & 8 & 4  & 2 & 75 & 10 & 20 & 73.2$\,/\,$-0.88 & 79.3$\,/\,$-0.55 & NA$\,/\,$-0.45 & 88.4$\,/\,$-0.24 & xx.x$\,/\,$xx.x & \textbf{94.6$\,/\,$-0.10} \\
    PP & RA & 9 & 2  & 4 & 30 & 5 & 25 & xx.x$\,/\,$-3.31 & xx.x$\,/\,$-2.98 & NA$\,/\,$-3.32 & x.xx$\,/\,$-3.18 & xx.x$\,/\,$xx.x & \textbf{xx.x$\,/\,$-2.93} \\
    ST & RA & 12 & 5  & 4 & 150 & 5 & 10 & xx.x$\,/\,$xx.x & xx.x$\,/\,$xx.x & xx.x$\,/\,$xx.x & xx.x$\,/\,$xx.x & xx.x$\,/\,$xx.x & \textbf{xx.x$\,/\,$xx.x} \\
    \bottomrule
\end{tabular}
\end{table*}
\end{comment}



%\subsection{Baselines}
%We compare \algname{} against two state-of-the-art IL approaches and two variations of our algorithm to validate our design choices.




%\subsection{Benchmarks}
%We now present the experimental setup for the various problem settings.
%\paragraph{Benchmarks} 
%We use the following three simulated scenarios to collect our training and testing data.
%Each demonstration contains both low-level action noise caused by the imperfect motion model and variations in the action labels caused by the probabilistic conditions in the ASP. 

    
%\noindent \textit{\textbf{Stop Sign (SS)}}: This is the one-dimensional example described in in \autoref{sec:overview}, where the demonstrator controls the vehicle to move to and stop at target locations.
    
%\noindent \textit{\textbf{Highway (HW)}}: This scenario uses the open-source simulation environment \textsc{highway-env}~\cite{Eleurent2021}, where a demonstrator controls a vehicle moving in a crowded multi-lane highway and needs to switch lanes to pass slower traffic. The high-level actions are 
%$\{\ha{FASTER}$, $\ha{SLOWER}$, $\ha{LANE\_LEFT},$ and $\ha{LANE\_RIGHT}\}$, \textit{accelerating, decelerating, turning left}, and \textit{turning right}. 
%The low-level actions are the amount of \textit{acceleration} and \textit{steering}. 
%Each demonstration lasts 100 time steps and contains about 10 high-level action transitions.
    %\item 
    
%\noindent \textit{\textbf{Merge (MG)}}: This setting is similar to \textit{Highway}, except that the robot is initially in the left-most lane, and instead of maneuvering around slower traffic, the expected behavior is to quickly and safely merge into the rightmost lane. This scenario uses the same high-level and low-level actions as \textit{Highway} but with a different, more aggressive motion model. 
%and demonstrations that reward more aggressive driving. 
%Each demonstration lasts 75 time steps and contains about 3-5 high-level action transitions. 
\begin{comment}
\noindent \textit{\textbf{Pick and Place (PP)}}: This scenario uses the open-source simulation environment \textsc{panda-gym}~\cite{Gallouedec2021}, modeled after the real-life Franka Emika Panda robot arm. In this experiment, we train a reinforcement learning agent using the Truncated Quantile Critics method (TQC), and use that to generate the expert trajectories, demonstrating the usage of \algname{} with less predictable error and approximate motion models rather than perfect ones. The low-level actions are desired displacement along the $x, y, $ and $z$ axes, as well as end-effector grasping control. We provide 5 demonstrations with 30 timesteps each.

\noindent \textit{\textbf{Stack (ST)}}: This setting also uses \textsc{panda-gym}, but the task is to stack two boxes in the correct order. This is the most complex environment, with five high-level labels, four low-level actions, and 5 demonstrations of 150 timesteps each.


%\blue{todo: we need to find papers that use the same environments and cite them here}


%\begin{itemize}
    %\item 
    \noindent
    \textit{\textbf{FitGreedy}}. This baseline represents the naive solution to the unlabeled demonstration problem in which each time step is labeled greedily with the action label whose likelihood is highest according to the motion model.
    %with action weights proportional to the likelihood given by the motion model. The final program is then synthesized based on these labels.

    \noindent
    \textit{\textbf{FitSmooth}}. This baseline instead labels the trajectories using a particle filter and the $\stx{randSwitch}(0.1)$ ASP. This baseline can be viewed as the first iteration of \algname{}, except that it does not employ incremental synthesis and directly searches over a much larger program space.
    %a heuristic prior that prefers maintaining the same state (with a 10\% chance of transitioning to another random label). This baseline can be viewed as the first iteration of \algname{}, except that it performs synthesis over a larger program space. Both \textit{FitGreedy} and \textit{FitSmooth} label high-level actions and perform synthesis over these high-level labels without embedding them inside an EM-loop.
    %\item 

    \noindent
    \textit{\textbf{BC}}. This behavior cloning baseline applies supervised learning to directly predict the low-level demonstrations. We use an LSTM with 64 hidden units and train it to predict the next low-level action conditioned on all previous states and low-level actions.
    
    % baseline uses a behavioral cloning approach~\cite{10.5555/3304652.3304697}. In the BC baseline we  apply supervised learning to the demonstrations to model low-level actions given state-action pairs directly. We designed an LSTM neural network with two dense hidden layers comprised of 64 sigmoid activation units each and trained it to predict the next low-level action.
    %\item 

    \noindent
    \textit{\textbf{BC+}}. This baseline extends \textit{BC} with access to the motion model. Instead of letting the LSTM directly output the low-level actions, in \textit{BC+}, we let the neural network output a distribution over all available high-level actions and then perform a weighted sum over the corresponding low-level actions (obtained by running the motion models). We then train \textit{BC+} in the same way as \textit{BC}.
    %\item 
    
%    \textit{\textbf{GAIL}}. This approach is the state-of-the-art imitation learning method for learning a policy directly from expert trajectories. It iterates between training a generator and discriminator neural network in a GAN-like manner, where the generator attempts to minimize discriminator accuracy, and the discriminator tries to maximize its ability to differentiate between expert and generator trajectories. Our generator consists of 3 fully connected layers, each one with 32 neurons; our discriminator is 2 layers of \fixme{?} neurons each. Similar to the \textit{BC} algorithm, \textit{GAIL} is not given high-level action labels or the motion model; however, similar to the RL setting, it can query a simulation with actions to generate its own samples. \fixme{???}
    %\item 

    \noindent
    \textit{\textbf{FitTruth}}. This baseline represents an idealized scenario where labels for all demonstrations are artificially provided, allowing synthesis to be performed directly on the labels. 
    %\item 
%\end{itemize}
\end{comment} 


\subsection{Common Setup}
%In the experiments below, for each scenario, we use the ground-truth probabilistic ASP to simulate 10 demonstrations to serve as the training data and an additional 20 demonstrations to serve as the test set. 
For each experiment, we use $M=2000$ particles to sample $N=50$ trajectories in the E step. To improve the M Step performance, we limit the number of transition examples to be at most 2000 and use the remaining examples as the validation set, which is used to calculate the final likelihood when deciding the best ASP. 
% Because the number of transition examples can be very large, we randomly split the examples into a training set, which we use to compute the M Step objective, and a validation set, used to calculate the final likelihood. 
%: we randomly pick 2000 examples to optimize over in the training set, and save the remaining examples to calculate the final likelihood. 
We use the L-BFGS optimizer over 4 random starting values to optimize the ASP parameters. All reported performance metrics are obtained by running each baseline 3 times and taking the best result.


    
\subsection{Accuracy Results} \jimmy{todo, if we're removing the table}

\begin{figure}
\includegraphics[width=0.46\textwidth]{figs/accuracy_results.pdf}
    \caption{Accuracy of \algname{} and baselines
    \jimmy{I like the graph, but GAIL and BC don't have a \% accuracy (no action labels), so we'll still have to include obs\_likelihood values somehow? Maybe in Table 1 -- I don't think the DemoLen, TrainSet, and TestSet are that important -- KIA: yes we are not done with the section yet. We will add obs ll for sure.}
    }
    \label{fig:la_demo_highway}
\end{figure}



In this section, we evaluate the synthesized ASPs in terms of their consistency with the ground-truth action labels and with the provided low-level demonstrations. We report the results in \autoref{tab:pct_accuracy}. The percentage of action labels that match the ground truth are shown in columns 2, 3, and 4 (except for \textit{BC}, which does not produce high-level labels), and we report the observation log likelihood of the low-level demonstrations (normalized over the number of time steps) in columns 5, 6, and 7. We find that \algname{} consistently outperforms the other baselines.
Our experiments also confirm our hypothesis that the accuracy of the synthesized policies improves as the iterative EM loop proceeds.
%
Under standard amounts of noise, it takes less than \jimmy{waiting for stack} iterations for \algname{} to converge to a policy for all benchmarks. \autoref{fig:loop_progress} visualizes the performance of the synthesized policy after each iteration of the EM loop in the \textit{Stop Sign} benchmark. 
%
Note that the accuracy trend in the training set is reflected in the test set results, indicating that our approach generalizes well to new data.
%and performs similarly to \textit{FitTruth}. Interestingly, we also found \algname{} outperforming \textit{FitTruth} in some cases. We hypothesize that this is because \textit{FitTruth} learns from only a single action label sequence and hence is more prone to overfitting. In contrast, our algorithm samples additional action label sequences in the E-step, which helps the M-step to generalize.

\begin{figure}
    % HIGH RES FIGURE: use this for the final version
%\includegraphics[width=0.42\textwidth]{figs/la-graph.png}

    % LOW RES FIG: use this temporariliy to speed up pdf compilation
%\includegraphics[width=0.44\textwidth]{figs/la-graph-low-res.png}
    \caption{An example low-level observation sequence predicted by \algname{} for the \textit{Merge} scenario. 
    }
    \label{fig:la_demo_highway}
\end{figure}

We visualize the low-level observations generated by the synthesized policy for the \textit{Merge} benchmark in \autoref{fig:la_demo_highway}. The top plot shows the demonstrated steering control (red) and the predicted trajectory (green). The bottom plot shows the demonstrated acceleration (blue) and the policy's prediction (yellow). We can see that the synthesized program closely follow the ground truth in both cases.
%
%Note that for the percent accuracy metric we artificially provide baseline labels; manually labeling trajectories in real life given the data would be tedious, time-consuming, and potentially less accurate compared to our approach. 




\begin{figure}
    \centering
    % HIGH RES FIGURE: sue this for the final version
%\includegraphics[width=0.38\textwidth]{figs/1D-target-emloop.png}

    % LOW RES FIG: use this temporariliy to speed up pdf compilation
%\includegraphics[width=0.38\textwidth]{figs/1D-target-emloop-low-res.png} 

    \caption{EM loop progress until convergence in the \textit{Stop Sign} setting. Results for the test set are similar to that of the training set, indicating that our approach generalizes well. %\fixme{replace with high res before submit}
    }
    \label{fig:loop_progress}
\end{figure}




\subsection{Impact of Noise}
\label{subsec:noise}

\begin{figure}
    \centering
%\includegraphics[width=0.43\textwidth]{figs/noise.png}
    \caption{Accuracy of baselines at varying levels of noise in the \textit{Merge} benchmark. Noise levels are scaled to fit the range $[0, 1]$ for presentation purposes.
%    \fixme{replace with high-res}
    }
    \vspace{-4mm}
    \label{fig:noise}
\end{figure}

In this section, we evaluate how the performance of each baseline changes as we vary the amount of actuation noise in the training data using the \textit{Merge} setting. The observation log likelihoods of the trajectories produced by all approaches are plotted in \autoref{fig:noise}. We find that all approaches decrease in performance as noise is increased; however, \algname{} consistently outperforms other baselines, indicating that it is robust against low-level noise. We also observe that with higher noise, \algname{} takes more iterations to converge. In the least noisy setting, it converges in 5 iterations, but in the noisiest setting, it requires 12 iterations. 

We find that \textit{FitSmooth} consistently outperforms \textit{FitGreedy}, demonstrating the importance of the E Step, even with a very basic ASP. Additionally, we note that \textit{BC+} significantly outperforms \textit{BC} when there are large amounts of noise, suggesting that having access to motion models defined by action labels provides useful inductive bias that helps overcome the noise in the data.

%When low-level actions are noisy, a purely data-driven approach performs poorly, indicating the importance of using a programmatic prior to guide the particle filter, even a simple one like \textit{$\asp^{(0)}$}.

\subsection{Importance of Probabilistic ASP}
A crucial component of \algname{} is its use of probabilistic programs to account for the inherent uncertainty in human demonstrations. %This approach generates distributions of high-level labels that provide guidance to the particle filter, as explained in previous sections. 
In this experiment, we compare this approach with LDIPS~\cite{ldips}, a state-of-the-art PIL approach that produces deterministic ASPs. We conducted a case study using the \textit{Stop Sign} benchmark. 
%An integral aspect of \algname{} is the use of \textit{probabilistic programs}, which captures the uncertainty inherent in the human demonstrations, and produces distributions of high-level labels that are used to guide the particle filter. 
%However, this necessitates the use of \textit{probabilistic program synthesis} which can effectively capture uncertainty near thresholds.
%To further motivate this design decision, we performed a case study in \textit{Stop Sign} benchmark using the state-of-the-art  ASP synthesizer, LDIPS~\cite{ldips}, which synthesizes deterministic robot policies. 


Directly integrating LDIPS into our algorithm would result in the immediate breakdown of the E Step since all trajectories would be identical. To avoid this, we first execute the synthesized deterministic ASP at each time step and then randomly switch the high-level label with a probability of 0.1, akin to the heuristic prior used in $\asp^{(0)}$.

The experiment yielded the following observations. First, we observed that the synthesized programs performed poorly, with $87.5\%$ accuracy and an average observation likelihood of $-1.403$. These scores fall significantly below the performance of \algname{} from \autoref{tab:pct_accuracy}. Second, the performance of LDIPS remains largely the same after each EM iteration, confirming our hypothesis that a deterministic program is insufficient for capturing label uncertainties. Lastly, LDIPS also exhibited another fundamental limitation---namely its inability to account for the proximity of each example to the threshold. Deterministic program synthesizers  maximize the number of satisfied examples regardless of their likelihood, which quickly leads to poor performance as the noise level becomes nontrivial.

% For instance, upon closer inspection of the synthesized program for the Stop Sign benchmark, we observed nonsensical expressions such as ${\stx{distTrv}(v_{\max},a_{\max})-\dns > -99.74 }$, which is useless since $\stx{distTrv}$ is only useful for negative acceleration values (recall that $0\!<\!a_{\max}$). 
% y using probabilistic program synthesis, our approach overcomes the above limitations and synthesizes a program which optimizes for total likelihood over all demonstrations.
%\begin{figure}[h]
%    \centering
%\includegraphics[width=0.5\textwidth]{figs/ldips.png}
%    \caption{Progress of EM loop using deterministic vs. probabilistic synthesis}
%    \label{fig:ldips}
%\end{figure}
\subsection{Qualitative Analysis}
In this section, we analyze programs that are synthesized by our algorithm. We find that in all  benchmarks, the synthesized programs contain conditions that are non-trivial and require multiple incremental synthesis steps. For example, we present the following program, which was synthesized in the \textit{Highway} setting for the transition $\ha{FASTER}$ $\rightarrow$ $\ha{LANE\_LEFT}$:
%
$$
 \begin{array}{ll}
\guard_{\ha{FASTER},\ha{LANE\_LEFT}} & = \stx{flp}(\stx{lgs}(x - f_x, -30.62, 1.78))  \\
&  \wedge\ \stx{flp}(\stx{lgs}(f_x - l_x, -4.92, -6.53)) \\ 
&  \wedge\ \stx{flp}(\stx{lgs}(r_x - l_x, 2.95, -1.67))
 \end{array}
$$
which translates to the condition ``if the vehicle's position $(x)$ is approaching the position of the vehicle in front $(f_x)$, and the position of the vehicle to the left $(l_x)$ is farther away than both the vehicle in front and the position of the vehicle to the right $(r_x)$, then turn left." 
We note that this complex program is beyond the scope of naive enumeration techniques, which would need to optimize well over one billion programs in our DSL to reach a program of this complexity. Such techniques are unable to synthesize this program on its own, much less be embedded inside an EM loop that requires many iterations of synthesis.


\subsection{Interpretability} \jimmy{to do}
Synthesizing a program over discrete high-level transitions also has the benefit of being interpretable and amenable to repair~\cite{idips}. We find that in our experiments, our approach performs the worst on transitions that have little to no data from the demonstrations. Take the \textit{Merge} setting as an example, which has no data for the $\ha{FASTER}$ $\rightarrow$ $\ha{LANE\_LEFT}$ transition. Consider the highest-noise setting in \autoref{subsec:noise}. \algname{} attempts to fit to a few noisy examples and incorrectly synthesizes the program $\stx{flp}(\stx{lgs}(l_{v_x}, 40.03, 77.10))$ for the transition $\ha{FASTER}$ $\rightarrow$ $\ha{LANE\_LEFT}$, where $l_{v_x}$ is the forward velocity of the vehicle to the left. Our approach makes it easy to alter programs; for example, in this case, we can simply remove this transition. The new program achieves an average log-likelihood of $-1.724$, an improvement from the standard \algname{} performance of $-1.869$. Other approaches generally do not have this benefit and cannot be confidently repaired in this simple manner. 
%In particular, we note that we cannot restrict the low-level actions, because multiple distinct high-level labels can map to the same low-level actions.

\begin{comment}
\subsubsection{Testing vs training performance (Generalization)? \fixme{if space}}
 4.1 Experimental setup (introduce all settings formally):
    - 1D-target: sequential, contains large swaths where a LA maps to different HA. Also inductively generalizes
    - 2D-merge: ideally, an environment where the ground-truth program is very complex, and we are able to synthesize a good estimate.
    - 2D-highway: randomized environment. randomized environment allows the algorithm to learn an inductively generalizing policy. Very noisy low-level actions allow our iterative method to shine
    - if time, ability to \textit{approximate} very complex programs that are not synthesizable directly
- interpretability: discuss ability to verify the program, ability to easily adjust, ability to easily restrict transitions if necessary. Note that in the merge case, you cannot restrict low-level actions because you can have left-turning motion without "turning left"
\end{comment}

